NeuroWeaver: An Autonomous Evolutionary Agent for Exploring the Programmatic Space of EEG Analysis Pipelines

Although foundation models have achieved remarkable success in general domains, applying them to electroencephalography (EEG) analysis is constrained by substantial data requirements and large parameter counts, which incur prohibitive computational costs and impede deployment in resource-constrained clinical environments. General-purpose automated machine learning frameworks are likewise ill-suited to this domain, since exploration within an unbounded programmatic space fails to incorporate essential neurophysiological priors and frequently yields neuroscientifically implausible solutions. We therefore propose NeuroWeaver, a unified autonomous evolutionary agent that generalizes across diverse EEG datasets and tasks by reformulating pipeline engineering as a discrete constrained optimization problem solved through large language model (LLM)-driven generation of executable code. A Domain-Informed Subspace Initialization confines the search to a neuroscientifically plausible manifold, while a Multi-Objective Evolutionary Optimization dynamically balances performance, novelty, and efficiency via self-reflective refinement. Across five heterogeneous benchmarks, NeuroWeaver synthesizes lightweight pipelines that outperform state-of-the-art task-specific methods on nearly all metrics and attain accuracy comparable to large-scale foundation models, even surpassing them on the HMC and Workload benchmarks with only $0.18$M and $0.011$M parameters, respectively.

==> tables/table_efficiency.tex <==
\begin{table}[htbp]
\centering
\caption{\textbf{Efficiency profile of the synthesized pipelines $s^*$ against the strongest task-specific baseline on each dataset.} Time-to-plateau denotes the cumulative wall-clock time at which the smoothed training loss first reaches $1.05$ times its final value over $30$ epochs under the native training recipe of each method. \textbf{Bold} marks the more efficient value within each (dataset, metric) pair.}\label{tab:efficiency}
\fontsize{8}{9.6}\selectfont
\setlength{\tabcolsep}{5pt}
\renewcommand{\arraystretch}{1.20}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{l l c c c c c c}
\toprule
\multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{Params (M)}} & \multicolumn{3}{c}{\textbf{Training (batch size 64)}} & \multicolumn{2}{c}{\textbf{Inference latency (ms)}} \\
\cmidrule(lr){4-6} \cmidrule(lr){7-8}
 &  &  & Step time (ms) & Peak mem (MiB) & Time-to-plateau (s) & bs $=$ 1 & bs $=$ 64 \\
\midrule
\multirow{2}{*}{\textsc{SEED}} & CNN-Transformer~\cite{peh2022transformer} & 3.20 & 27.3 & 515 & 223 & 11.9 & 15.3 \\
 & NeuroWeaver & \textbf{0.374} & \textbf{1.93} & \textbf{244} & \textbf{43.8} & \textbf{0.36} & \textbf{0.40} \\
\addlinespace[2pt]\cmidrule(l){1-8}\addlinespace[2pt]
\multirow{2}{*}{\textsc{HMC}} & CNN-Transformer~\cite{peh2022transformer} & 3.20 & 21.9 & 1021 & 689 & 4.31 & 4.90 \\
 & NeuroWeaver & \textbf{0.176} & \textbf{2.59} & \textbf{195} & \textbf{150} & \textbf{0.45} & \textbf{0.50} \\
\addlinespace[2pt]\cmidrule(l){1-8}\addlinespace[2pt]
\multirow{2}{*}{\textsc{TUEV}} & ContraWR~\cite{yang2023self} & 1.58 & 4.91 & 491 & 206 & 1.32 & 2.11 \\
 & NeuroWeaver & \textbf{1.20} & \textbf{3.51} & \textbf{410} & \textbf{62.2} & \textbf{0.53} & \textbf{0.79} \\
\addlinespace[2pt]\cmidrule(l){1-8}\addlinespace[2pt]
\multirow{2}{*}{\textsc{TUSL}} & ContraWR~\cite{yang2023self} & 1.58 & \textbf{8.02} & \textbf{895} & \textbf{0.72} & 1.31 & \textbf{3.00} \\
 & NeuroWeaver & \textbf{0.463} & 39.4 & 5300 & 5.1 & \textbf{0.30} & 8.91 \\
\addlinespace[2pt]\cmidrule(l){1-8}\addlinespace[2pt]
\multirow{2}{*}{\textsc{Workload}} & FFCL~\cite{li2022motor} & 2.41 & 17.3 & 734 & 13.0 & 5.77 & 6.57 \\
 & NeuroWeaver & \textbf{0.011} & \textbf{5.18} & \textbf{557} & \textbf{2.6} & \textbf{0.23} & \textbf{0.80} \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}


==> tables/table_hyperparams.tex <==
\begin{table}[htbp]
\centering
\caption{\textbf{Search hyperparameters of the MOEO engine.} The reported values are used across all experiments and are organized by the two roles that the hyperparameters serve. Tree Expansion controls how the solution tree is grown along its draft, improvement, and debugging branches; UCT Exploration governs the decay schedule of the exploration constant in the UCT selection criterion.}\label{tab:hyperparams}
\fontsize{8}{9}\selectfont
\setlength{\tabcolsep}{6pt}
\renewcommand{\arraystretch}{1.2}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{>{\raggedright\arraybackslash}p{0.27\textwidth} >{\raggedright\arraybackslash}p{0.5\textwidth} c}
\toprule
\textbf{Hyperparameter} & \textbf{Description} & \textbf{Value} \\
\midrule
\rowcolor{gray!15}\multicolumn{3}{c}{\textit{Tree Expansion}} \\
\midrule
Root draft count                        & Initial draft solutions sampled at the root before any refinement begins. & 5 \\
Improvement children per parent         & Maximum improvement children spawned from a single executable parent.       & 3 \\
Repair attempts per buggy parent        & Maximum repair children emitted from a single buggy parent. & 1 \\
Maximum debug chain depth               & Maximum length of a chain of consecutive repair attempts along the same lineage; once exceeded, the buggy lineage is no longer selected for further repair. & 20 \\
Maximum consecutive improvement failures & Consecutive non-improving refinements tolerated on a branch before the branch is terminated. & 3 \\
Metric improvement threshold            & Minimum primary-metric gain required to register an executable child as an improvement. & $10^{-4}$ \\
\midrule
\rowcolor{gray!15}\multicolumn{3}{c}{\textit{UCT Exploration}} \\
\midrule
Decay schedule                          & Schedule applied to the exploration constant of the UCT selection criterion. & piecewise \\
Initial exploration constant            & Initial value of the UCT exploration constant, set to the conventional $\sqrt{2}$. & $1.414$ \\
Exploration lower bound                 & Asymptotic lower limit toward which the exploration constant decays.        & $0.5$ \\
Decay step size                         & Step-wise decrement applied to the exploration constant during the decay phase. & $0.01$ \\
Phase boundary ratios                   & Fractions of the iteration budget that delimit the constant-exploration, decay, and exploitation phases of the piecewise schedule. & $(0.3,\,0.7)$ \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}


==> tables/table_matched_budget.tex <==
\begin{table}[htbp]
\centering
\caption{\textbf{Matched-budget comparison against automated ML-engineering agents on HMC, TUEV, and TUSL.} All systems share the same backbone LLM and a budget of 200 code-synthesis iterations; we report mean $\pm$ standard deviation over three random seeds. AIDE on TUSL is reported as N/A because none of its 200 iterations yields a script that completes end-to-end execution. \underline{Underlined}: strongest baseline per cell; \textcolor{blue}{blue}: NeuroWeaver surpasses every baseline.}\label{tab:matched_budget}
\fontsize{8}{9}\selectfont
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.05}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{l ccc ccc ccc}
\toprule
\multirow{2}{*}{System} &
\multicolumn{3}{c}{HMC} & \multicolumn{3}{c}{TUEV} & \multicolumn{3}{c}{TUSL} \\
\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}
& Balanced Acc. & Cohen’s Kappa & Weighted F1
& Balanced Acc. & Cohen’s Kappa & Weighted F1
& Balanced Acc. & Cohen’s Kappa & Weighted F1 \\
\midrule
\rowcolor{gray!15}\multicolumn{10}{c}{\textit{ML Engineering Agents}} \\
\midrule
AIDE~\cite{jiang2025aide}
& 0.6615 $\pm$ 0.0538 & 0.5699 $\pm$ 0.1198 & 0.6784 $\pm$ 0.0963
& \underline{0.4653} $\pm$ 0.0108 & \underline{0.2591} $\pm$ 0.1129 & 0.5129 $\pm$ 0.2127
& N/A & N/A & N/A \\
ML-Master~\cite{liu2025ml}
& \underline{0.7834} $\pm$ 0.0007 & \underline{0.7098} $\pm$ 0.0020 & \underline{0.7748} $\pm$ 0.0016
& 0.3579 $\pm$ 0.0092 & 0.2460 $\pm$ 0.0538 & \underline{0.5860} $\pm$ 0.0955
& \underline{0.5480} $\pm$ 0.0103 & \underline{0.1349} $\pm$ 0.0096 & \underline{0.3636} $\pm$ 0.0228 \\
\midrule
\rowcolor{gray!15}\multicolumn{10}{c}{\textit{Domain-Informed ML Engineering Agent (Ours)}} \\
\midrule
NeuroWeaver
& \textcolor{blue}{0.7862} $\pm$ 0.0006 & \textcolor{blue}{0.7160} $\pm$ 0.0003 & \textcolor{blue}{0.7794} $\pm$ 0.0004
& \textcolor{blue}{0.4887} $\pm$ 0.0057 & \textcolor{blue}{0.4400} $\pm$ 0.0203 & \textcolor{blue}{0.7205} $\pm$ 0.0163
& \textcolor{blue}{0.7138} $\pm$ 0.0117 & \textcolor{blue}{0.2206} $\pm$ 0.0281 & \textcolor{blue}{0.4373} $\pm$ 0.0329 \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}


==> tables/table_seed_hmc.tex <==
\begin{table}[htbp]
\centering
\caption{\textbf{Performance comparison on the SEED and HMC benchmarks.} Balanced Accuracy, Cohen $\kappa$, and Weighted F1 are reported as mean $\pm$ standard deviation over three independent runs. \underline{Underlined} entries mark the best result within each method category, while \textcolor{blue}{blue} indicates that NeuroWeaver surpasses the strongest task-specific baseline; the two model sizes correspond to SEED and HMC, respectively.}\label{tab2}
\fontsize{8}{9}\selectfont
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.05}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{lc ccc ccc}
\toprule
\multirow{2}{*}{Method} & \multirow{2}{*}{Model Size} &
\multicolumn{3}{c}{SEED} & \multicolumn{3}{c}{HMC} \\
\cmidrule(lr){3-5}\cmidrule(lr){6-8}
& & Balanced Acc. & Cohen’s Kappa & Weighted F1
  & Balanced Acc. & Cohen’s Kappa & Weighted F1 \\
\midrule
\rowcolor{gray!15}\multicolumn{8}{c}{\textit{Task-specific Methods}} \\
\midrule
SPaRCNet~\cite{jing2023development} & 0.79M & 0.5596 $\pm$ 0.0244 & 0.3464 $\pm$ 0.0372 & 0.5585 $\pm$ 0.0297 & 0.4756 $\pm$ 0.1109 & 0.3147 $\pm$ 0.1315 & 0.4108 $\pm$ 0.1310 \\
ContraWR~\cite{yang2023self} & 1.6M  & 0.6106 $\pm$ 0.0078 & 0.4220 $\pm$ 0.0129 & 0.6137 $\pm$ 0.0085 & 0.4242 $\pm$ 0.0541 & 0.2340 $\pm$ 0.0554 & 0.2987 $\pm$ 0.0288 \\
CNN-Transformer~\cite{peh2022transformer} & 3.2M & \underline{0.6161} $\pm$ 0.0384 & \underline{0.4262} $\pm$ 0.0601 & \underline{0.6150} $\pm$ 0.0463 & \underline{0.6573} $\pm$ 0.0141 & \underline{0.5961} $\pm$ 0.0105 & \underline{0.6896} $\pm$ 0.0065 \\
FFCL~\cite{li2022motor} & 2.4M & 0.5808 $\pm$ 0.0322 & 0.3732 $\pm$ 0.0462 & 0.5743 $\pm$ 0.0402 & 0.4427 $\pm$ 0.0702 & 0.2542 $\pm$ 0.0654 & 0.2902 $\pm$ 0.0485 \\
ST-Transformer~\cite{song2021transformer} & 3.5M & 0.5479 $\pm$ 0.0091 & 0.3261 $\pm$ 0.0169 & 0.5505 $\pm$ 0.0091 & 0.2559 $\pm$ 0.0141 & 0.0503 $\pm$ 0.0183 & 0.1428 $\pm$ 0.0122 \\
\midrule
\rowcolor{gray!15}\multicolumn{8}{c}{\textit{Pretrained Foundation Models}} \\
\midrule
BIOT~\cite{yang2023biot} & 3.2M & 0.7097 $\pm$ 0.0024 & 0.5682 $\pm$ 0.0051 & 0.7134 $\pm$ 0.0027 & 0.6862 $\pm$ 0.0041 & 0.6295 $\pm$ 0.0113 & 0.7091 $\pm$ 0.0147 \\
LaBraM-Base~\cite{jiang2024large} & 5.8M & \underline{0.7318} $\pm$ 0.0019 & \underline{0.5994} $\pm$ 0.0031 & \underline{0.7354} $\pm$ 0.0021 & \underline{0.7286} $\pm$ 0.0101 & \underline{0.6812} $\pm$ 0.0073 & \underline{0.7554} $\pm$ 0.0024 \\
NeuroLM-B~\cite{jiangneurolm} & 254M & 0.5554 $\pm$ 0.0075 & 0.3393 $\pm$ 0.0117 & 0.5599 $\pm$ 0.0068 & 0.6737 $\pm$ 0.0050 & 0.6188 $\pm$ 0.0057 & 0.7126 $\pm$ 0.0034 \\
\midrule
\rowcolor{gray!15}\multicolumn{8}{c}{\textit{Agent System}} \\
\midrule
NeuroWeaver & 0.37M/0.18M   & \textcolor{blue}{0.6211} $\pm$ 0.0058 & \textcolor{blue}{0.4397} $\pm$ 0.0087 & \textcolor{blue}{0.6246} $\pm$ 0.0058 & \textcolor{blue}{0.7862} $\pm$ 0.0006 & \textcolor{blue}{0.7160} $\pm$ 0.0003 & \textcolor{blue}{0.7794} $\pm$ 0.0004 \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}


==> tables/table_tuev_tusl.tex <==
\begin{table}[htbp]
\centering
\caption{\textbf{Performance comparison on the TUEV and TUSL benchmarks.} Balanced Accuracy, Cohen $\kappa$, and Weighted F1 are reported as mean $\pm$ standard deviation over three independent runs. \underline{Underlined} entries mark the best result within each method category, while \textcolor{blue}{blue} indicates that NeuroWeaver surpasses the strongest task-specific baseline; the two model sizes correspond to TUEV and TUSL, respectively.}\label{tab3}
\fontsize{8}{9}\selectfont
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.05}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{lc ccc ccc}
\toprule
\multirow{2}{*}{Method} & \multirow{2}{*}{Model Size} &
\multicolumn{3}{c}{TUEV} & \multicolumn{3}{c}{TUSL} \\
\cmidrule(lr){3-5}\cmidrule(lr){6-8}
& & Balanced Acc. & Cohen’s Kappa & Weighted F1
  & Balanced Acc. & Cohen’s Kappa & Weighted F1 \\
\midrule
\rowcolor{gray!15}\multicolumn{8}{c}{\textit{Task-specific Methods}} \\
\midrule
SPaRCNet~\cite{jing2023development} & 0.79M & 0.4161 $\pm$ 0.0262 & \underline{0.4233} $\pm$ 0.0181 & \underline{0.7024} $\pm$ 0.0104 & 0.4185 $\pm$ 0.0452 & 0.1399 $\pm$ 0.0799 & 0.3500 $\pm$ 0.0968 \\
ContraWR~\cite{yang2023self} & 1.6M & \underline{0.4384} $\pm$ 0.0349 & 0.3912 $\pm$ 0.0237 & 0.6893 $\pm$ 0.0136 & \underline{0.5857} $\pm$ 0.0662 & \underline{0.3567} $\pm$ 0.0968 & \underline{0.5458} $\pm$ 0.0798 \\
CNN-Transformer~\cite{peh2022transformer} & 3.2M & 0.4087 $\pm$ 0.0161 & 0.3815 $\pm$ 0.0134 & 0.6854 $\pm$ 0.0293 & 0.3575 $\pm$ 0.0151 & 0.0306 $\pm$ 0.0179 & 0.2235 $\pm$ 0.0251 \\
FFCL~\cite{li2022motor} & 2.4M & 0.3979 $\pm$ 0.0104 & 0.3732 $\pm$ 0.0188 & 0.6783 $\pm$ 0.0120 & 0.3819 $\pm$ 0.0688 & 0.0628 $\pm$ 0.0888 & 0.2120 $\pm$ 0.0786 \\
ST-Transformer~\cite{song2021transformer} & 3.5M & 0.3984 $\pm$ 0.0228 & 0.3765 $\pm$ 0.0306 & 0.6823 $\pm$ 0.0190 & 0.4000 $\pm$ 0.0329 & 0.0860 $\pm$ 0.0449 & 0.3793 $\pm$ 0.0459 \\
\midrule
\rowcolor{gray!15}\multicolumn{8}{c}{\textit{Pretrained Foundation Models}} \\
\midrule
BIOT~\cite{yang2023biot} & 3.2M & 0.5281 $\pm$ 0.0225 & 0.5273 $\pm$ 0.0249 & 0.7492 $\pm$ 0.0082 & 0.5758 $\pm$ 0.0303 & 0.2012 $\pm$ 0.0212 & 0.2394 $\pm$ 0.0040 \\
LaBraM-Base~\cite{jiang2024large} & 5.8M & \underline{0.6409} $\pm$ 0.0065 & \underline{0.6637} $\pm$ 0.0093 & \underline{0.8312} $\pm$ 0.0052 & \underline{0.7625} $\pm$ 0.0131 & \underline{0.6407} $\pm$ 0.0304 & \underline{0.7614} $\pm$ 0.0210 \\
NeuroLM-B~\cite{jiangneurolm} & 254M & 0.4560 $\pm$ 0.0048 & 0.4285 $\pm$ 0.0048 & 0.7153 $\pm$ 0.0028 & 0.6734 $\pm$ 0.0436 & 0.5107 $\pm$ 0.0617 & 0.6743 $\pm$ 0.0394 \\
\midrule
\rowcolor{gray!15}\multicolumn{8}{c}{\textit{Agent System}} \\
\midrule
NeuroWeaver & 1.2M/0.46M & \textcolor{blue}{0.4887} $\pm$ 0.0057 & \textcolor{blue}{0.4400} $\pm$ 0.0203 & \textcolor{blue}{0.7205} $\pm$ 0.0163 & \textcolor{blue}{0.7138} $\pm$ 0.0117 & 0.2206 $\pm$ 0.0281 & 0.4373 $\pm$ 0.0329 \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}


==> tables/table_workload.tex <==
\begin{table}[htbp]
\centering
\caption{\textbf{Performance comparison on the binary Workload benchmark.} Balanced Accuracy, AUC-PR, and AUROC are reported as mean $\pm$ standard deviation over three independent runs. \underline{Underlined} entries mark the best result within each method category, while \textcolor{blue}{blue} indicates that NeuroWeaver surpasses the strongest task-specific baseline.}\label{tab4}
\fontsize{9}{11}\selectfont
\setlength{\tabcolsep}{10pt}
\renewcommand{\arraystretch}{1.2}
\begin{adjustbox}{width=0.9\textwidth,center}
\begin{tabular}{l c ccc}
\toprule
\multirow{2}{*}{Method} & \multirow{2}{*}{Model Size} &
\multicolumn{3}{c}{Workload} \\
\cmidrule(lr){3-5}
& & Balanced Acc. & AUC-PR & AUROC \\
\midrule
\rowcolor{gray!15}\multicolumn{5}{c}{\textit{Task-specific Methods}} \\
\midrule
SPaRCNet~\cite{jing2023development} & 0.79M & 0.5977 $\pm$ 0.0071 & 0.6638 $\pm$ 0.0314 & 0.6717 $\pm$ 0.0172 \\
ContraWR~\cite{yang2023self} & 1.6M  & 0.6966 $\pm$ 0.0332 & 0.7668 $\pm$ 0.0408 & 0.7685 $\pm$ 0.0317 \\
CNN-Transformer~\cite{peh2022transformer} & 3.2M & 0.5793 $\pm$ 0.0230 & 0.5306 $\pm$ 0.0459 & 0.5663 $\pm$ 0.0349 \\
FFCL~\cite{li2022motor} & 2.4M & \underline{0.7069} $\pm$ 0.0197 & \underline{0.7823} $\pm$ 0.0099 & \underline{0.7857} $\pm$ 0.0234 \\
ST-Transformer~\cite{song2021transformer} & 3.5M & 0.6103 $\pm$ 0.0056 & 0.5716 $\pm$ 0.0071 & 0.6375 $\pm$ 0.0078 \\
\midrule
\rowcolor{gray!15}\multicolumn{5}{c}{\textit{Pretrained Foundation Models}} \\
\midrule
BIOT~\cite{yang2023biot} & 3.2M & \underline{0.6655} $\pm$ 0.0665 & \underline{0.7189} $\pm$ 0.0722 & \underline{0.7342} $\pm$ 0.0536 \\
LaBraM-Base~\cite{jiang2024large} & 5.8M & 0.6609 $\pm$ 0.0204 & 0.7174 $\pm$ 0.0234 & 0.7272 $\pm$ 0.0165 \\
NeuroLM-B~\cite{jiangneurolm} & 254M & 0.6172 $\pm$ 0.0113 & 0.5824 $\pm$ 0.0080 & 0.6253 $\pm$ 0.0160 \\
\midrule
\rowcolor{gray!15}\multicolumn{5}{c}{\textit{Agent System}} \\
\midrule
NeuroWeaver & 0.011M   & \textcolor{blue}{0.7391} $\pm$ 0.0439 & \textcolor{blue}{0.8436} $\pm$ 0.0373 & \textcolor{blue}{0.8403} $\pm$ 0.0361 \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}

